On the Robustness of Language Guidance for Low-Level Vision Tasks: Findings from Depth Estimation

Recent advances in monocular depth estimation have been made by incorporating natural language as additional guidance. Although yielding impressive results, the impact of the language prior, particularly in terms of generalization and robustness, remains unexplored. In this paper, we address this gap by quantifying the impact of this prior and introduce methods to benchmark its effectiveness across various settings. We generate "low-level" sentences that convey object-centric, three-dimensional spatial relationships, incorporate them as additional language priors and evaluate their downstream impact on depth estimation. Our key finding is that current language-guided depth estimators perform optimally only with scene-level descriptions and counter-intuitively fare worse with low level descriptions. Despite leveraging additional data, these methods are not robust to directed adversarial attacks and decline in performance with an increase in distribution shift. Finally, to provide a foundation for future research, we identify points of failures and offer insights to better understand these shortcomings. With an increasing number of methods using language for depth estimation, our findings highlight the opportunities and pitfalls that require careful consideration for effective deployment in real-world settings

==> preamble.tex <==
\usepackage[x11names]{xcolor}
\definecolor{courage}{HTML}{FF8833}
\definecolor{truth}{HTML}{0000DD}
\definecolor{earth}{HTML}{008800}

\newcommand\Ri{{\color{courage} \texttt{\bf R1}}}
\newcommand\Rii{{\color{truth} \texttt{\bf R2}}}
\newcommand\Riii{{\color{earth} \texttt{\bf R3}}}
% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\usepackage[hang,para]{footmisc}
\setlength{\footnotemargin}{0mm}
\usepackage[skip=1pt,indent=0pt]{parskip}


